Statistical and computational thresholds for the planted $k$-densest sub-hypergraph problem

In this work, we consider the problem of recovery a planted $k$-densest sub-hypergraph on $d$-uniform hypergraphs. This fundamental problem appears in different contexts, e.g., community detection, average-case complexity, and neuroscience applications as a structural variant of tensor-PCA problem. We provide tight \emph{information-theoretic} upper and lower bounds for the exact recovery threshold by the maximum-likelihood estimator, as well as \emph{algorithmic} bounds based on approximate message passing algorithms. The problem exhibits a typical statistical-to-computational gap observed in analogous sparse settings that widen with increasing sparsity of the problem. The bounds show that the signal structure impacts the location of the statistical and computational phase transition that the known existing bounds for the tensor-PCA model do not capture. This effect is due to the generic planted signal prior that this latter model addresses.

==> sections/introduction.tex <==
High dimensional inference problems play a key role in recent machine learning and data analysis applications. Typical scenarios exhibit problem dimensions that are comparable to the sample size, hence precluding effective estimation with no further structure imposed on the underlying signal, such as low rank or sparsity. Examples of such problems include sparse mean estimation, compressive sensing, sparse phase retrieval, low-rank matrix estimation, community detection, planted clique and densest subgraph recovery problems.

In this work we study the problem of recovery a \emph{planted} $k$-densest sub-hypergraph on $h$-uniform hypergraphs over $n$ nodes recently introduced in \cite{corinzia2019}. This is the \emph{planted} version of the classical $k$-densest subgraph \cite{chlamtac2016densest}, informally defined as follows. The \emph{planted} solution consists of a set of $k$ randomly chosen nodes among the total of  $n$ nodes. The weights of all $\binom{n}{h}$ hyperedges~\footnote{Recall that in an $h$-uniform hypergraph we have one hyperedge for each subset of $h$ nodes, with $h=2$ being the standard undirect graph.} \emph{inside the planted solution} have some initial \emph{bias}, the others have zero bias. After some Gaussian \emph{noise} is added to these initial weights, we would like to recover the planted solution  given only these noisy observations. 
\begin{quote}
	\emph{Under what conditions is it \emph{possible} to recover the planted solution? \\
		What about computationally \emph{efficient} algorithms for this task?}
\end{quote}
In the simpler \emph{graph} setting the problem is closely related to detecting a core structure in community detection, it resembles the well-known planted clique problem, and other community detection models such as  the stochastic block model (SBM). Recent work also suggest that the $k$-densest subgraph problem is related to long term memory mechanism in the brain \cite{legenstein2018long}.  The more general \emph{hypergraph} version  is closely related to the so-called \emph{tensor} Principal Component Analysis (tensor PCA). Higher order interactions among nodes is also rather natural in several applications, including modeling brain regions \cite{gu2017functional, wang2012naive, zu2016identifying} and in computer vision applications \cite{jolion2012graph}. 

Our goal is to understand the \emph{information-theoretic} and \emph{computational} algorithmic limits for this class of recovery problems, thereby establishing the regimes for which algorithms have the ability to recover a hidden structure or signal from noisy measurements and partial information.
In particular, we are interested in the existence of the so called \emph{computational-to-statistical gaps} and whether the \emph{hypergraph parameter} $h$ plays a role. 
For a start, consider the two extremes $h=1$ and $h = k$, where the maximum likelihood estimator (MLE) is \emph{computationally efficient} though for \emph{different} reasons:
\begin{itemize}
	\item For $h=k$ the solutions are  statistically \emph{independent} (like in the Random Energy Model  \cite{derrida1981random}). The maximum likelihood estimator (MLE) can be implemented by searching exhaustively through all $\binom{n}{k}=\binom{n}{h}$ solutions, which is computationally efficient since $\binom{n}{h}$ is the input size. 
	\item  For $h=1$ exhaustive search through all $\binom{n}{k}$ solutions is clearly inefficient, unless $k$ is constant. Nonetheless simply selecting greedily the $k$ nodes with highest weights implements efficiently the MLE. Unlike the previous case, the solutions are statistically \emph{dependent}.
\end{itemize}
Therefore, in both these extreme cases there is \emph{no computational-to-statistical gap}, while their information-theoretic nature is very different. The case $h=1$ can be considered \emph{easier} from the pure information-theoretic point of view, since the analysis of recoverability conditions (whether the MLE succeeds)   boils down to analyzing $N=\binom{n}{h}$ \emph{independent} Gaussian random variables. The presence of \emph{dependencies} between solutions makes the analysis of the information-theoretic boundary conditions significantly more complex, even for $h=k$.

We are interested in the \emph{non-extreme} cases (the spectrum $1 < h \leq  k \leq n$), where most of the  practical and theoretical applications arise. These are also the most challenging cases since they present both challenges: information-theoretical due to \emph{dependencies} and algorithmic since the MLE is \emph{not} computationally efficient in general. In particular, we shall focus on the \emph{sparse} regime $k \ll n$ which, in several recovery problems, seems to be the major source of computational-to-statistical gaps. We mainly consider $k \approx n^\alpha$ with arbitrary $\alpha\in (0,1)$ constant (though some of our results extend to the full spectrum).  
%
%
%
%Analysing these extremes yields insight on the information structure of the solution space. For $h=k$ the problem has the highest \emph{localization}, i.e., there is \emph{only one biased} solution and all other solutions are \emph{unbiased} and statistically \emph{independent} (see the REM =Random Energy Model \cite{derrida1981random}). At the opposite extreme, for $h=1$, in addition to the planted solution, \emph{several} other partially overlapping solutions are \emph{biased}. In other words, for $h=1$, the problem exhibits some statistical \emph{dependencies} between solutions, which become more prominent for large $h$ (e.g., for $h = o(N)$). A second reason for investigating different values of $h$, are algorithmic issues. Dependencies between solutions and hence the localization property in the solution space render computationally efficient algorithms information theoretically possible (in principle). To illustrate this, consider the following scenarios:
%\begin{itemize}
%\item For $h$ and $k$ very close to each other ($h = k - c_0$ with $c_0$ being a constant), exhaustive search through all $\binom{N}{k}$ solutions is both efficient and unavoidable since solutions are localized and (almost) statistically \emph{independent}: the input size is $\binom{N}{h}$, and exhaustive search requires inspecting  $\binom{N}{k}=poly( \binom{N}{h})$ solutions.
%%and finding the optimum is equivalent to search through all these $\binom{N}{h}=poly( \binom{N}{h})$ edge weights.
%\item For $h=1$, exhaustive search through all $\binom{N}{k}$ solutions is clearly inefficient, i.e., $\binom{N}{k}$ is exponentially larger then the input size $\binom{N}{h} = N$. Nonetheless the structure of the solution space is simple and selecting the $k$ nodes with highest weights is efficient and optimally solves the problem.
%\item The intermediate sparse regime for $1 \ll h \ll k \ll N$ reveals insights into the information structure of sub-hypergraph recovery. In this regime the solution space can be again exponentially larger then the input size. In this regime, algorithms have to address the information theoretical localization effect in the solution space. i.e., two solutions that do not share any parameter are statistically independent.
%\end{itemize}

\subsection{Contributions}
We study the problem of recovery a \emph{planted} $k$-densest sub-hypergraph on $h$-uniform hypergraphs over $n$ nodes. We consider the version in which the planted solution (``signal'') is perturbed by  \emph{Gaussian} noise, as in the closely related tensor PCA problem (see below).  
For this natural problem above, we provide novel information-theoretic and algorithmic recovery thresholds on the \emph{signal-to-noise ratio (SNR)} necessary and sufficient to recover the planted solution in the sparse regime $k \approx n^\alpha$ with $\alpha \in (0,1)$ constant. The signal-to-noise ratio is intuitively defined as follows. 
All $\binom{k}{h}$ hyperedges inside the planted part have an initial positive \emph{bias} $\beta$, and therefore the ``total signal'' given by the planted solution is $\binom{k}{h}$. 
Since the noise added to each hyperedge is normally distributed $\sim \Gaussian(0,1)$, it is convenient to define the  ``total noise'' as   $\sqrt{\binom{k}{h} 2 k \log n} \sim \sqrt{\binom{k}{h} 2\log \binom{n}{k}}$, which intuitively incorporates the fact that we have $\binom{n}{k}$ solutions each of them with variance  (noise) $\sqrt{\binom{k}{h}}$  -- for more intuition on the logarithm see Remark~\ref{rem:SNR} below.
This leads to the \emph{scale-normalized} SNR defined as ``total signal/total noise'':
\begin{align}
\label{eq:rescaling}
\gamma \equiv  \beta \sqrt{\frac{\binom{k}{d}}{k}\cdot \frac{1}{2\log p}}.
\end{align}
 The above normalization is introduced in order to incorporate the problem parameters $p, k, d$ so that the \emph{information-theoretic recoverability} thresholds corresponds to a \emph{finite $\gamma$} (see next paragraph and Remark~\ref{rem:SNR} below). Note that both $k$ and $d$ may depend on $p$, that is, we  consider  $k=k_p$ and $d_p$ for  $n\rightarrow \infty$. We should also emphasize that for constant $\gamma$, the signal $\beta$  depends on $p, k$ and $d$ and, in particular, $\beta = \beta(p) =\Theta\left(\sqrt{\frac{{2k\log p}}{\binom{k}{p}}}\right)$. 

\paragraph{Tight information theoretic bounds for recovery.} 
We show that recoverability using (computationally-unbounded) estimators is impossible or possible, when the scale-normalized SNR $\gamma$ in \cref{eq:rescaling} is below or above the following two constants:
\begin{align}\label{eq:bounds:intro}
\begin{split}
\gamma_{LB} =& \begin{cases}
\sqrt{1-\alpha_k} & \text{for any $h \in \omega(1)$} \\
\sqrt{1-\alpha}/2 & \text{in general}
\end{cases} \\ 
\gamma_{UB} =& \sqrt{1+2\alpha} + \sqrt{\alpha} \ ,
\end{split}
\end{align}
where $\alpha\in (0,1)$ is a constant satisfying $k \approx n^\alpha$. Specifically, we prove the following: 

%\begin{quote}
\emph{\textbf{Theorem (informal)} 
For  $\gamma<\gamma_{LB}$, exact recovery is \emph{impossible} regardless of which estimator (algorithm) we use, while for  $\gamma > \gamma_{UB}$ the exact recovery is possible via the (computationally intractable) maximum likelihood estimator. 
}
%\end{quote}

We stress that  the bounds are essentially tight since they refer to a \emph{scale-normalized} SNR $\gamma$ which contains the leading factors (see \cref{eq:rescaling}).  We indeed observe that, if we cast the problem in the tensor PCA formulation, the bounds that can be obtained from the literature  are far from optimal for our problem. Our bounds also improve drastically over the known bounds for this problem \cite{corinzia2019} (see \Cref{sec:prior_bounds_from_us} for a detailed comparison). 
The upper bound is based on an union bound analysis, which actually provides thresholds for \emph{partial recovery} as well. For example, a threshold $1+\sqrt{\alpha}$ is enough to recover any constant fraction of the planted solution (see \Cref{th:UB} for the exact bounds). The lower bound is a major technical contribution as it requires to deal with non-trivial \emph{dependencies} between solutions (partial overlaps). For this we provide different proofs which employ the following arguments. The first proof uses a  generalized Fano's inequality and packing/covering suitably adapted to our problem; The second proof uses recent tail bounds for maximum of Gaussian r.v. with bounded correlation, also combined with the packing/covering argument. 
\paragraph{New algorithmic results based on approximate message passing (AMP)} For many high dimensional statistical estimation problems this class of algorithms represent the best known technique, e.g., planted clique \cite{deshpande2015finding}, dense and sparse PCA on both matrix and higher order tensors \cite{richard2014statistical, lesieur2017constrained, lesieur2017statistical}. Recent work \cite{Kikuchi-hierarchy} suggest that a hierarchy of such AMP algorithms may actually match the performance of the best known efficient algorithms.

We provide an heuristic derivation of AMP together with a state evolution analysis for our problem as a generalization of the tensor PCA AMP algorithm with non-factorizable prior distribution and obtain the following non-trivial \emph{computationally-efficient} threshold: 
$$\gamma_c^{AMP} = \sqrt{\frac{1}{2 e} \left(\frac{n}{k}\right)^{h-1} \frac{1}{h(h-1)\log n}}\ .$$
Intuitively, for $k \approx n^\alpha$ and by ignoring low order terms, the above bound corresponds to $\gamma_c^{AMP} \approx \sqrt{n^{(1-\alpha)(h-1)}/(h(h-1)\log n)}$.

%\begin{theorem}[Main Result]
%	\label{th:main-informal}
%	There exist an upper bound $\gamma_{UB}$ and a lower bound $\gamma_{LB}$ which determine whether recovery is possible or not possible, respectively: \\ 
%	\textbf{Upper bound:} For $\gamma > \gamma_{UB}^{(k')}$ it is \emph{possible} to perform a $(k'+1)$-partial recovery; for $\gamma>\gamma_{UB} \equiv \gamma_{UB}^{(k-1)}$ it is possible to perform exact recovery. These thresholds depend on the problem parameters ($N,k,k',h$) as follows:
%	\begin{equation}
%	\label{eq:UB_partial}
%	\gamma_{UB}^{(k')} \equiv \sqrt{1+\beta_0-2\beta_0'+\beta_0''} + \sqrt{\beta_0-\beta_0'+\beta_0''}
%	\end{equation}
%	\begin{equation}
%	\label{eq:UB_exact}
%	\gamma_{UB} \equiv \sqrt{1+ 2\beta_0} + \sqrt{2\beta_0}
%	\end{equation}
%	\textbf{Lower bound:} For $\gamma < \gamma_{LB}$, exact recovery is \emph{impossible}. Specifically, the lower bound depends on the parameters ($N,k,h$) as follows:
%	\begin{equation}
%	\label{eq:LB}
%	\gamma_{LB} \equiv \max \left\{\sqrt{\frac{1}{h}}, \sqrt{\frac{1 - \beta_0 - \epsilon}{2}\frac{k_\star}{k}} \right\}  
%	\end{equation}
%	for any constant $\epsilon > 0$ and any function $k_\star$ such that $\binom{k_*}{h}/\binom{k}{h} \rightarrow 0$.
%\end{theorem}

\subsection{Related work}
Tensor PCA is a very closely related problem to ours, and the new results also suggest an interesting comparison with the known bounds \cite{richard2014statistical,richard2014statistical,hopkins2015tensor,montanari2016limitation,jagannath2020statistical,arous2020algorithmic, perry2020}:
1) Applying the tensor PCA bounds ``black-box" to our problem yields bounds that are far from optimal in most of the cases (see for example the upper and lower bounds given in \Cref{sec:TPCA}). The reason is that our problem imposes a ``combinatorial'' structure on the planted vector (a restricted prior) which tensor PCA does not have. The bounds must take into account this structure in the form of both parameters  $k$ and $h$.
2) While approximate message passing does not have a provable guarantee for ``generic''  tensor PCA, in our problem we are able to obtain a provable (algorithmic) SNR threshold; Moreover, this algorithm can be also experimentally tested to verify some `robustness' property when it is initialized with the (correct) planted solution: Below our information-theoretic threshold, even with this initialization, it fails to return the planted solution (while above the information-theoretic threshold) it succeeds (when provided with this side-information).

Finally, we noticed that tensor PCA has yet a subtle difference. In tensor PCA, the estimator has more observations available in the form of ``diagonal entries/self-loops'' (for the simple matrix case $h=2$, in tensor PCA we can also observe the ``diagonal'' elements $W_{ii}$). This means that algorithms for tensor PCA may not work for our problem (our experiments of AMP in this regard confirm that for some range of values these extra information is indeed important). 
%Moreover, having access to these ``additional diagonal observations'' may yield \emph{faster} estimators directly from our bounds (if  the SNR in our problem allows some estimator to recover for some $h'<h$, then the same estimator could just read these $\binom{n}{h'}\ll \binom{n}{h}$ values of the tensor and recover as well). 

 
Our problem is closely related to the well studied \emph{tensor PCA} and variants of the stochastic block model (SBM) studied in community detection. Here one seeks to recover some ``dense'' community hidden in a random graph. Notable examples include the \emph{planted clique problem} \cite{barak2016nearly}, its ``relaxed'' version known as the \emph{$k$-densest subgraph} \cite{brennan18}, and extensions to uniform \emph{hypergraphs} \cite{ke2020exact}. All these works deal with \emph{unweighted} (Bernulli) random \emph{graph} models.

The problem considered here, instead, deals with the \emph{weighted} (Gaussian) model, where edges can assume different (continuous) weights. These formulations are notoriously more powerful in many applications, and they are sometimes referred to as weighted stochastic block model (WSBM) in community detection \cite{aicher2014learning,peixoto2018nonparametric}. Moreover, we consider the case of \emph{hypergraphs}, which strictly generalizes the graph setting ($h=2$) to higher order interactions \cite{Benson163,grilli2017higher,ke2019community}.
This results in a tensor PCA with a restricted prior to encode the solutions ($k$-densest sub-hypergraphs). Restricted priors are also studied in \cite{perry2020}, where the authors provide tight threshold for (weak) recoverability for different problems and for ``generic'' (spherical) prior. Unlike ours, their restricted priors result in a moderate change in the information-theoretic threshold.

 Different statistical and computational thresholds have been observed also in the problem of \emph{sparse} PCA \cite{deshpande2014information, berthet2013complexity} and in \emph{some} versions of the stochastic block model (SBM) \cite{abbe2016exact,mossel2015consistency,abbe2015community,chen2014statistical}. Statistical and computational thresholds are still unknown for various SBM generalizations, including the \emph{weighted} SBM (WSBM) \cite{aicher2014learning,peixoto2018nonparametric} and the SBM on $h$-uniform hypergraph (hSBM) \cite{chien2018community,ghoshdastidar2014consistency}.
For the WSBM, information-theoretic results are only known for \emph{dense} regimes \emph{and} by adding some additional restrictions ($h=2$ \cite{jog2015information} and $h=4$ \cite{kim2017community}, where in both works the planted part consists two or more communities of equal size $k = \Theta(n)$).
Spectral algorithms have been studied on \emph{unweighted} hypergraphs \cite{ghoshdastidar2014consistency,ghoshdastidar2017consistency}. 


%%% shorter version %%%%%%
Recent developments focused on recovery conditions for the spike Wigner model \cite{krzakala2016mutual,dia2016mutual,barbier2019adaptive,aubin2020spiked,perry2020}, SBM \cite{zdeborova2016statistical,barbier2019mutual}, generalized linear models \cite{barbier2019optimal}. These approaches have been mainly applied to dense scenarios -- roughly speaking, the case $k=\rho n$ for constant $\rho$. The extension to sparse scenarios have been developed recently in \cite{barbier2020all}.
Further work relate the computationally hard regimes to the so-called overlap gap property (OGP) \cite{gamarnik2019overlap,gamarnik2019overlap,OGP-densesubgraph, arous2020free}.
A recent work on tensor PCA \cite{niles2020all} considers the
minimum mean square error (MMSE) estimator. Their work shows that, under rather general conditions, there is a sharp  critical threshold for the MMSE estimator in the sparse regimes; for our problem, after a proper rescaling, this  yields a sharp threshold $\gamma^{\MMSE} = \sqrt{1-\alpha}$  for this estimator which corresponds a \emph{weak} recovery condition (positive correlation).


==> sections/related_work.tex <==
The first and probably most widely studied planted model in literature is the \emph{planted clique problem}, where a clique of size $k$ is hidden in a Erd\"os-R\'enyi random graph of size $n$. This problem exhibits a \emph{statistical-computational gap} \cite{steinhardt2017does}, meaning that recovery of the planted clique is information-theoretic possible for size $k \geq 2 \log_2 n$, while the best known polynomial-time algorithms require $k = \Omega(\sqrt{n})$ \cite{barak2016nearly}. It is an open problem to assess whether the regime $k=o(\sqrt{n})$ is indeed intractable. Many variations of this problem have been introduced, allowing for generic values of the ER parameter, for random deletion of edges in the planted clique, and for weighted edges (i.e.\ planted densest subgraph problem \cite{arias2013community}). 

 Similar statistical and computational thresholds have been observed also in the problem of sparse principal component analysis \cite{deshpande2014information, berthet2013complexity} and in some versions of the stochastic block model (SBM). The standard SBM exhibits no gap, with matching statistical and computational thresholds that have been found recently for the symmetric \cite{abbe2016exact,mossel2015consistency} and the non-symmetric \cite{abbe2015community} model. 
The SBM extension to multi-community detection (also known as planted clustering problem) shows instead statistical-computational gaps \cite{chen2014statistical}. Statistical and computational thresholds are still unknown for various SBM generalizations, like weighted-SBM (WSBM) \cite{aicher2013adapting,aicher2014learning,peixoto2018nonparametric} and SBM on $h$-uniform hypergraph (hSBM) \cite{chien2018community,ghoshdastidar2014consistency}. Information-theoretic results are given for the following problems: homogeneous WSBM with equally sized communities \cite{jog2015information},  for the spectral algorithms respectively on uniform \cite{ghoshdastidar2014consistency} and non-uniform hSBM  \cite{ghoshdastidar2017consistency}, in \cite{kim2017community} for the homogeneous equally sized community WSBM on hypergraphs \cite{kim2017community}, and in \cite{corinzia2019} for the non-equally sized communities WSBM on hypergraphs. \\ 
Information-theoretic results are given in \cite{jog2015information} for the homogeneous WSBM with equally sized communities, in \cite{ghoshdastidar2014consistency,ghoshdastidar2017consistency} for the spectral algorithms respectively on uniform and non-uniform hSBM, in \cite{kim2017community} for the homogeneous equally sized community WSBM on hypergraphs and in \cite{corinzia2019} for the non-equally sized communities WSBM on hypergraphs. 

Recent work in statistical physics gives us a better understanding of the nature of the information-theoretic and computational thresholds. Planted inference models are mapped to related disordered physical systems (e.g.\ spin glass, Potts and Mattis models  \cite{stein2013spin}) such that the statistical and computational thresholds are mapped to the phase transitions of these systems \cite{nishimori2001statistical,iba1999nishimori}. 
The hard phase of planted inference problems is conjectured to correspond to the spin-glass phase of related disorder systems, that is typically characterized by exponentially many clusters of solutions with close energy values and large energy walls between them \cite{monasson1997statistical,mezard2005clustering,achlioptas2006solution}, while the impossible and the easy regimes are mapped respectively to the paramagnetic and the ferromagnetic phases. 
This line of research was inspired by the seminal work done on error correcting codes using p-spin glass models \cite{sourlas1989spin,rujan1993finite,kinouchi1992optimal} and its Random Energy Model (REM) limit \cite{Derrida1980,talagrand2003spin,Bovier2006CUP}, with recent developments focused on recovery conditions for the spike Wigner model \cite{krzakala2016mutual,dia2016mutual,barbier2018rank,barbier2019adaptive,aubin2019spiked}, stochastic block model \cite{zdeborova2016statistical,barbier2019mutual}, generalized linear models \cite{barbier2019optimal}. These approaches have been mainly applied to dense scenarios, with the structure of the measurement imposed by the low dimensionality of the signal. The extension to sparse scenarios have been developed recently in \cite{barbier20190} (see also  \cite{bandeira2018notes} for a survey).
Recent work employ the so-called overlap gap property (OGP) \cite{OGP-submatrix,OGP-p-spin,OGP-densesubgraph}.

Our setting differs from the problems studied in these works in few key aspects which makes these results not directly applicable to our problem.  Though the model in \cite{OGP-p-spin} is also defined on $h$-uniform hypergraphs, there the feasible solutions are the vectors $v \in \{-1,+1\}^n$, and the associated weight is defined as $S(v) \equiv \sum_{i_1i_2\cdots i_h} W_{i_1i_2\cdots i_h} \cdot  v_{i_1}v_{i_2}\cdots v_{i_h}$. This means that (i) we cannot express that feasible solutions are subsets of $k$ nodes and (ii) the weight is different from ours since every hyperedge contributes either positively or negatively depending on the ``parity'' of $v_{i_1}v_{i_2}\cdots v_{i_h}$. Our formulation in \cref{eq:weight-def} instead corresponds to $v \in \{0,1\}^n$ with $\sum_i v_i =k$. The special case of our setting restricted to $h=2$ (graphs) is considered in \cite{OGP-submatrix} where the authors consider the ``non-sparse'' regime $k = \rho n$ for some constant $\rho\in (0,1)$ and provide nearly tight bounds for recovery. In this setting, the OGP mentioned above appears in a range where the SNR is slightly above the information-theoretic recovery threshold. Finally, the planted $k$-densest subgraph is studied in \cite{OGP-densesubgraph}, though under the \emph{Bernulli} (``unweighted'') random graph model where each hyperedge is present with some constant probability $p$ depending whether the hyperedge is inside the planted part or not $(p>1/2$ and $p=1/2$, respectively). The authors of \cite{OGP-densesubgraph} show an OGP based on an \emph{upper bond} on the actual overlap between the planted solution and the outcome of the MLE; such an upper bound is an ``optimized'' union bound, and the authors base their analysis on the conjecture that such an upper bound is indeed tight. The same problem in \cite{OGP-densesubgraph}, planted $k$-densest subgraph in the Bernulli random graph model, is also studied in  \cite{brennan18}, where the authors provide reductions between several planted problems.  

%\begin{problem}[Symmetric Tensor PCA]
%	Given an input tensor $\bT=\tau \cdot v^{\otimes h} +\bA$, where $v\in R^n$ is an arbitrary unit vector, $\tau\geq 0$ is the signal-to-noise ratio, and $\bA$ is a random noise tensor with iid standard Gaussian entries, recover the signal $v$ approximately. Moreover, the noise tensor is \textit{symmetric} and thus so is the input tensor as well, that is, $\bA_{\indperm} = \bA_{\ind}$ and  $\bT_{\indperm} = \bT_{\ind}$ for any permutation $\pi$.
%\end{problem}	
%	
%\begin{problem}[Planted $k$-Densest Sub-Hypergraph] 
%This problem is a variant of symmetric tensor PCA in which we impose the following additional structure:
%	\begin{enumerate}
%		\item\label{cond:distinct}We consider only the ${n \choose k}$ entries with \emph{distinct} indices, that is, $\bT_{\ind}=0$ whenever $i_a=i_b$ for some $a$ and $b$.
%		\item The vector $v$ encodes a planted $k$-Subgraph and thus has \emph{exactly} $k$ entries equal to $1/\sqrt{k}$, and all other entries are equal to $0$.
%	%	\item Both the noise and the input tensor are \emph{symmetric}, that is, $\bA_{\indperm} = \bA_{\ind}$ and  $\bT_{\indperm} = \bT_{\ind}$ for any permutation $\pi$.
%		
%	\end{enumerate}
%\end{problem}	
%
%
%\begin{remark}[Impact of diagonal entries -- \Cref{cond:distinct}]
%	Dropping Condition~\ref{cond:distinct} leads to the variant in which we make the substitution ${n \choose h} \mapsto n^h$ in \Cref{cond:distinct} above.
%\end{remark}
%	
%		\begin{remark}[Rescalings]
%		Different papers consider different rescaling of the signal-to-noise ratio (SNR):
%		\begin{align} 
%		\bT=\beta \cdot v^{\otimes h} +\bA && 	\bA_{\ind} \sim \Gaussian(0,1/(n(h-1)!))  &&  &&  && SNR:~\beta~\cite{richard2014statistical} \\
%		\bT=\beta' \cdot v^{\otimes h} +\bA && 	\bA_{\ind} \sim \Gaussian(0,2/(n\cdot h!))  &&  &&  && SNR:~\beta'~\cite{NIPS2015_5719} \\
%		\bT=\tau \cdot v^{\otimes h} +\bA && 	\bA_{\ind} \sim \Gaussian(0,1)  &&  &&  && SNR:~\tau~\cite{hopkins2015tensor} \\
%		\bT=\lambda \sqrt{n}\cdot v^{\otimes h} +\bA && 	\bA_{\ind} \sim \Gaussian(0,1)  &&  &&  && SNR:~\lambda ~\cite{jagannath2018statistical,arous2018algorithmic}\\
%		\bT=\mu \sqrt{k^h} \cdot v^{\otimes h} +\bA && 	\bA_{\ind} \sim \Gaussian(0,1)  &&  &&  &&SNR:~\gamma = \mu \sqrt{\frac{{k \choose h}}{k}\cdot \frac{1}{2\log n}} 
%		\end{align}
%		and therefore
%		\begin{align}\label{eq:SNR-rescaling}
%		\tau = \beta \sqrt{n \cdot (h-1)!} = \beta' \sqrt{n \cdot \frac{h!}{2}} = \lambda \sqrt{n} && \beta = \beta'\frac{h}{2} &&
%			\tau = \mu \sqrt{k^h} \\
%			 \gamma = \tau \sqrt{\frac{{k \choose h}}{k^{h+1}}\cdot \frac{1}{2\log n}} 
%		\end{align}
%		The information-theoretic bounds read as follows:
%		\begin{align}
%			\text{lower bound  \cite{richard2014statistical}:} && \beta \leq \sqrt{\frac{h}{10}} && \tau \leq \sqrt{\frac{n \cdot h!}{10}} && \gamma \leq \sqrt{\frac{n\cdot h! {k \choose h}}{k^{h+1} }\frac{1}{20\log n}}\\
%			\text{upper bound  \cite{richard2014statistical}:} &&\beta \geq \sqrt{h \log h} && \tau \geq \sqrt{n \cdot h!\log h} && \gamma \geq \sqrt{\frac{n\cdot h! {k \choose h}}{k^{h+1} }\frac{\log h}{2\log n}}
%		\end{align}
%		The algorithmic upper bounds provided by sum-of-squares algorithms \cite{hopkins2015tensor} are (for any constant $h\geq 3$):
%		\begin{align}
%		\tau^{SOS} \geq n^{h/4}\log (n)^{1/4}/\epsilon &&  && \gamma^{SOS} \geq \sqrt{\frac{n^{h/2}{k \choose h}}{k^{h+1}}\frac{1}{2\epsilon^2\log (n)^{1/2}}} 
%		\end{align}
%		where $\epsilon k$=loss in our setting and thus  $\epsilon = 1/k$.
%\end{remark}
%	
%	
%\begin{remark}[non-closed form thresholds]
%\begin{align}
%	\beta^{2nd}_h \equiv \inf_{q\in(0,1)} \sqrt{-\frac{1}{q^h}\log (1-q^2)} && \text{detection with eigenvalues} && \cite{NIPS2015_5719} \\
%	\lambda_c \equiv \sup\left\{\lambda\geq 0 \mid \sup_{t\in[0,1)} f_\lambda(t) \leq 0\right\}	&& \text{detection = positive correlation} && \cite{jagannath2018statistical} \\
%	f_\lambda(t) = \lambda^2 t^h + \log(1-t) + t \nonumber 
%\end{align}
%\end{remark}
